Bitcoin Payment-channels for Resource Limited IoT Devices

Resource-constrained devices are unable to maintain a full copy of the Bitcoin Blockchain in memory. This paper proposes a bidirectional payment channel framework for IoT devices. This framework utilizes Bitcoin Lightning-Network-like payment channels with low processing and storage requirements. This protocol enables IoT devices to open and maintain payment channels with traditional Bitcoin nodes without a view of the blockchain. Unlike existing solutions, it does not require a trusted third party to interact with the blockchain nor does it burden the peer-to-peer network in the way SPV clients do. The contribution of this paper includes a secure and crypto-economically fair protocol for bidirectional Bitcoin payment channels. In addition, we demonstrate the security and fairness of the protocol by formulating it as a game in which the equilibrium is reached when all players follow the protocol.

==> Notes/UseCase.tex <==


\begin{figure*}
\centering
\procedure{\todo{REDO this whole thing}   Real-time Data Reporting and Billing Protocol}{%
\textbf{Smart Meter} \< \< \textbf{Utility Provider}  \pclb
\pcintertext[dotted]{ Channel Open } \\
KGen(), \sigma_{SM}, \sigma_{UP}, G, tx\_id_{SM}  \<\< KGen(), \sigma_{SM}, \sigma_{UP}, G, tx\_id_{UP} \\
\< \sendmessageright*{pk_{SM}} \< \\
\< \sendmessageleft*{pk_{UP}} \< \\
\text{compute } in_{INIT} = in(\sigma_{SM},rd_1'(pk_0,sk_0),tx\_id_{SM}) \< \< \text{compute } in_{INIT} = in(\sigma_{UP},rd_1'(pk_0,sk_0),tx\_id_{UP}) \\
T_{FUND} = T_{FT}(in_{INIT},) \\
\<\<\<\pclb
\pcintertext[dotted]{ Real-time Payment and Measurement } \\
\<\< \text{compute } \Vec{p} = \left<p_1,p_2,...,p_n \right> \\
\< \sendmessageleft*{\Vec{p}} \< \\
\text{measure } \Vec{m} = \left<m_1,m_2,...,m_n \right> \<\< \\
\text{compute } B = \sum_{i=1}^{n} (m_i p_i T_C) \<\< \\
\< \sendmessageright*{\Vec{m}, \textbf{ConUp}(B)} \< \\
\< \sendmessageleft*{P} \< \pclb
\pcintertext[dotted]{ Channel Close } \\
\<\<\< \\
\<\<\< \\
\<\<\< \\
\<\<\< \\
}
\end{figure*}









%The Funding Transaction $T_{FT}$ is a tuple consisting of inputs\footnote{There may need to be multiple inputs from a party in order to total the correct number of funds agreed upon. For simplicity we assume here only one input is needed from each party.} from the smart meter and utility provider and an output to a 2-of-2 multisignature as well as change outputs (unless the parties with to use all the redeeming funds in the channel): 
%\

==> Notes/origional.tex <==
%\IEEEPARstart{T}{he} 
%last decade has seen vast deployments of advanced metering infrastructure (AMI) technology across the globe. 
%Smart meters  deployed in residential and industrial locations provide accurate and timely energy usage information to the utility providers that are used for billing, and ensuring correct grid operations.
%Operations of modern power grids are improved by increasing the situational awareness of the grid operators.
%Real-time measurement data is used by the utility company to better measure power flows and use real-time energy data to better allocate grid resources.
%Furthermore, electricity demand is dynamic with peak usage during the day and low points during off hours.
%The utility provider must allocate and procure resources to meet the demand which results in complex energy markets between power generation, transmission, distribution, and end users.
%
%Having detailed usage information allows parties to engage in more complex pricing models such as time-of-use, conditional and real-time pricing that encourage stabilization of energy usage through efficient markets.
%Frequent meter readings in AMI networks can can provide insightful information about the end users behavior which may be valuable to the utility company at expense to users' privacy. 
Decentralized trustless value ledgers in the form of blockchains have gained increasing traction as trust-less value transfer protocols.
Blockchains have caused widespread disruption across many domains including finance, insurance, internet of things, advertisement, entertainment, and even smart grid infrastructure.
%The novelty of blockchain technology is the design of a cryptoeconomic consensus algorithm which relaxes the assumption that some number of agents are honest to economically rational.
%This creates a state that as long as participants value money (or digital cash) they will behave in a way that results in their own best interest i.e., highest profits.
By design, blockchain consensus ensures correct operation of a decentralized public database which records users account balances.
Blockchain technology allows for users to transfer value to other users without the help of trusted third parties such as PayPal or Visa.

The energy sector has seen a number of proposals designed to leverage blockchain's decentralization and trustless systems \cite{blockchain:energy:1,blockchain:energy:2,blockchain:energy:3,blockchain:energy:4,blockchain:energy:5,blockchain:energy:7,blockchain:energy:8}. 
In \cite{blockchain:energy:2}, the authors provide an overview of blockchain integration and projects within the energy sector including markets, operations and stability and security of the grid.
Furthermore energy companies such as BAS Nederland, Enercity, Elegant, and Marubeni all accept Bitcoin payments \cite{blockchain:energy:9}. companies such as PowerLedger (\url{https://powerledger.io/}), and LO3 Energy (\url{https://lo3energy.com/}), offer peer-to-peer renewable energy marketplaces. 

The main advantage of blockchain is that it is a trust-less value transfer protocol that is securely maintained through decentralized participants.
However blockchain technology does not solve all problems, specifically blockchains suffer from limited scalability due to their decentralized nature.
Additionally the limited scalability can drive up the cost of using the blockchain network through high fees.
In our work we focus on using blockchain payment channels which enables scalability.


The remaining paper is organized as follows: Section \ref{background} provides background on AMI functionality and billing as well as blockchain as a value transfer protocol. Section \ref{design} presents our design and analysis of utilizing blockchain as a value transfer protocol while Section \ref{related-work} discusses blockchain developments within the context of the electric power grid. Finally Section \ref{conclusion} concludes this paper. 


\section{Background}
\label{background}

%\subsection{Smart Meters}
%AMI systems are deployed at end users homes and businesses and have several benefits including real-time usage reporting, and automatic meter reading for billing.
%Automated meter reporting systems were designed to record the periodic usage and report the value to the billing center.
%Initially this prevented the need for the utility to manually read each meter by physically observing the value.
%The utility bill would then be calculated from the reported value.
%While automatic meter reading has an upfront cost to deployment, they redeem their value as meter reading can take place automatically and be electronically transmitted to the utility provider saving the utility costs.
%In this work we analyze real-time payment for energy usage which would allow for automatic billing reducing costs for the utility provider further.
%
%The electric power grid has undergone a transition to accommodate bidirectional flow of electricity generated from distributed energy resources as well as operate the grid more efficiently.
%This smarter grid relies on an secure and efficient communication network between end users and energy suppliers, as well as on measurement and management devices within the energy infrastructure. 
%AMI networks enable utility providers to obtain real-time measurement values to aid in grid operations.
%
%Smart grid communication networks are composed of diverse communication mediums including power line carrier, cellular communication, TCP/IP Ethernet, and wireless mesh networks.


\todo{USE CASE elaborate on types of communication
%
\subsubsection{pricing models}
\cite{AMI:pricing:mit}
\cite{AMI:pricing:appE}
\cite{AMI:pricing:elecr}
\cite{AMI:pricing:EEcon}
%
\ 
%
aggregated, CPT, prepayment (iec 62055-41:2018) etc. 
%
}
\subsection{blockchain}
Blockchain technology at its core is an immutable public digital ledger containing transactions.
The novelty of blockchain is its ability to unequivocally agree on the state of the ledger in a decentralized setting. 
Through the process of \textit{mining}, the global state of the blockchain advances. 

The Bitcoin blockchain \cite{BTC:whitepaper} provides the ability to send transactions which consist of inputs, outputs, and rules governing the redemption of the outputs.
Inputs to transactions map to the source of the funds (a previous transaction) while the outputs represent the destination of the transaction value.
The governing rules included in the transaction dictate how the recipient of the transaction is able to spend the received value in the future.
A common rule is for the recipient to prove ownership of a private key associated with the destination address in the transaction. 
However more detailed rules can be expressed to provide more complicated value redemption logic.

In general, an input to a new Bitcoin transaction is the output of an unspent previous transaction along with a script that redeems the previous transactions output while the  output of the new transaction provides the recipient and a script telling the recipient how to redeem the values. 
Since the blockchain is an immutable public database, transactions can not be revoked and the total of all unspent transaction outputs represent the current state of the Blockchain.
Thus there is no concept of users or accounts included in the Bitcoin Blockchain.

Transactions are organized into blocks which remain pending until a partial pre-image is found for the sha-256 
%\footnote{In implementation the pre-image is hashed twice with sha-256.} 
 hash algorithm which meets a specific criteria quantified as the blockchain's difficulty. 
This difficulty is a dynamic variable that corresponds to the processing power of participants working to add new blocks and transactions into the blockchain. 
The result of this process maintains that on average new blocks are added to the blockchain every 10 minutes.
In alternative blockchain implementations the target block interval varies, eg. 15 seconds in Ethereum \cite{ETH:whitepaper}.
This interval is important to note because until a transaction is included in a block it is not considered verified by the blockchain network.
Furthermore, due to the consensus algorithm that governs the blockchain, there may be a temporary fork where there are multiple valid blocks at the same height.
A block is only valid if it is part of the longest blockchain.
Confidence of immutability grows exponentially in relation to the depth of the block ie. number of proceeding blocks. 
The original Bitcoin white paper \cite{BTC:whitepaper} provides a more detailed analysis however one heuristic used in practice is 6 blocks (about 60 minutes)\cite{BTC:wiki}.

\section{Real-time Payment Design}
\label{design}

We base our design off the assumptions listed below. 
\begin{itemize}
    \item Underlying blockchain is secure and has availability with the assumptions made in \cite{BTC:whitepaper,BTC:lightning}.
    \item Smart meters are trusted hardware that support cryptographic  operations of hash function, ECDSA key generation and storage.
    \item Smart meters and utility company have access to the blockchain peer-to-peer network.
\end{itemize}

\subsection{On-Chain Transactions}
In this section we explore the implications of using the Bitcoin blockchain for real-time AMI payments.
We can formulate the problem by generalizing the AMI communication protocol into three parts: (1) meta data that identifies the meter ID, location, configuration, etc., (2) measurement data as a fixed point vector, and (3) the real-time payment.

One approach to using Bitcoin to pay in real time for electricity usage would be to encode the measurement data and the meta data of the existing AMI protocol into existing fields in a Bitcoin transaction. 
The utility provider can monitor the blockchain and look for transactions that it is involved in and parse the measurement data and meta data and verify correct payment. 
While the blockchain is public, the transaction values and inputs/outputs will be public which can leak aggregate data about the smart meters energy usage even if the smart meter data is encrypted.
Additionally, storage on the blockchain is expensive and does not meet our real-time objectives. 
This is similar to the approach proposed for storing phasor measurement units and other data sources in \cite{blockchain:energy:8} which suffers from data storage and IO limits.

In AMI networks it is more favorable not to broadcast the information public but rather to include the receipt of a Bitcoin transaction into an existing AMI data reporting protocol. 
A transaction identifier or receipt is the hashed value of the transaction that is stored in the Bitcoin merkle tree data structure within the blockchain.
Transaction identifiers can uniquely identify a transaction and provide the necessary information for the utility provider to look up the transaction on the blockchain to verify payment. 
The cost of transferring Bitcoin is determined by the market through a transaction fee. 
This fee is dependant on the frequency of the data reporting interval as well as the number of other transactions included at a given time. 

The fee associated with sending a transaction on the blockchain is proportional to the size of the transaction in bytes. 
The size of the transaction however is not directly related to the amount of value being transferred, it is dependant on the history of the unspent coins used in the transaction and the new outputs, including directions for redeeming the outputs.
The formula to calculate \textit{basic} transactions is
$$ 148  i + 34  o + 10 \pm i$$
where $i$ is the number of inputs and $o$ is the number of outputs. 
The number of bytes for the input is because a public key and a signature need to be included to redeem the coins from the previous transaction. 
The number of bytes for per output correspond to the hash of the public key needed to redeem the funds. 
The plus-minus part comes from the fact that key length is not a fixed size
The number of inputs into the transaction will likely be small since the quantity of value transferred will be small and likely from the same source transaction while the outputs should be 2. 
One output is the utility provider and the second a refund address for any change in the transaction.
The minimum transaction size will be 226 bytes
for the end-consumer to send payment alongside the metering data.
As an example, if Alice has received 2 \bitcoin from Bob last week and 3.5 \bitcoin from Bob yesterday and she wishes to send 5 \bitcoin to Carol now, the transaction format would take in the two unspent transactions from Bob as inputs and create two outputs, one to Carol for 5 \bitcoin and one to herself for 0.5 \bitcoin as change. 
The total transaction size is $148 \times 2 + 34 \times 2 + 10 \pm 2 = 374 \pm 2$ bytes.

Figure \ref{fees} shows the USD value of fees on from Feb 2018 to June 2018 of transactions included on the Bitcoin Blockchain. The data was collected from the Bitcoin Blockchain and parsed using the BlockSci \cite{btc:block:sci} toolkit.
Figure \ref{sizes} shows the average transaction size in Bytes of transactions included in the same time range. 
The transaction sizes typically range from 500 to 1000 Bytes after mid-March.

\begin{figure}
\centering
\includegraphics[scale=.425]{2018_fees.pdf}
\caption{Average fee per transaction in USD }
\label{fees}
\end{figure}

\begin{figure}
\centering
\includegraphics[scale=.425]{2018_sizes.pdf}
\caption{Average transaction size in Bytes }
\label{sizes}
\end{figure}

Because the transaction fees are much greater than the payments themselves this solution is not feasible.
While frequent real-time transactions for energy usage are not possible, a single transaction per month does not incur outrageous fees. 
However that is equivalent to the existing billing strategy.
Another method to reduce fees is to use an alternative blockchain that has larger block sizes or more frequent blocks.
Although alternative blockchains can have weaker security, greater price volatility that 
%A single monthly transaction is closer to the existing billing solutions which 
doesn't satisfy our goals in this work.
Instead we propose a protocol using off-chain payment channels that can provide real-time payment but do not incur large fees with frequent posting to the blockchain.

\subsection{Off-Chain Bitcoin Transactions}
Bitcoin's Forth-like scripting language enables more complex functionality by placing conditions on the redeeming of transaction outputs. 
For example, time locks can be used on transactions and transaction outputs to place temporal restrictions on transactions.
Time locks can be both relative and absolute and can prevent a transaction output from being spent until after a certain time. 
Time locks are one of the most important building blocks in off-chain Bitcoin Transactions such as in the Bitcoin Lightning Network \cite{BTC:lightning}.
Multisignatures can require multiple keys to spend a transaction output.
One use case for multisignatures is joint savings accounts where both parties need to agree to make a transaction. 
%Multisignatures
%A Hashed TimeLock Contract (HTLC) is a type of contract that builds off timelock and hashlock scripting primitives. 
%HTLCs are contracts that require additional information in order to make the transaction valid. 
%The timelock requires a temporal attribute to become valid while the hashlock requires a hash function pre-image to validate a transaction.
Time lock contracts include primitives \cite{BTC:wiki} such as
\begin{itemize}
    \item \texttt{nLockTime} specifies the minimum height of the blockchain that a transaction can be included in.
    \item \texttt{checkLockTimeVerify} requires that the blockchain be at a certain height for the output of an already included transaction to be spent.
    \item \texttt{Relative lockTime} places restrictions on the inclusion of an input to a new transaction based on the time the input was included in the previous transaction. ie., restricting the time sent BTC can be sent again.
    \item \texttt{CheckSequenceVerify} is used to provide a relative time that the output of a valid transaction becomes valid after inclusion in a block. 
    \item \texttt{Multisig} can be used to require $m-\text{of}-n$ signatures to become valid.
\end{itemize}
\texttt{nLockTime} and \texttt{Relative Locktime} are corresponding counterparts for absolute and relative time respectively for inclusion into the blockchain while  \texttt{CheckLockTimeVerify} and \texttt{CheckSequenceVerify} are counterparts for absolute and relative time respectively for making outputs of a valid transaction spendable.

Hashlocks on the other-hand provide encumbrance on the outputs of transaction that require as input some secret value that is the pre-image to some hash functions output.
Upon unlocking the hashlock, all other hashlocks with the same secret value are also unlocked due to the secret value being recorded on the blockchain.

The combination of hashlocks and timelocks can create timed hashlock contracts (HTLCs) which can be used to put Bitcoin transactions 'off-chain' through what is called L2 or layer 2 scaling solutions such as the Lightning Network \cite{BTC:lightning}, Duplex micropayment channels\cite{BTC:duplex}, and Raiden \cite{ETH:Raiden}. 
Our protocol uses \texttt{CheckSequenceVerify} and \texttt{Multisig} for payment channels similar to Lightning Network Transactions.
Off-chain transactions are properly formatted Bitcoin transactions that are deferred from being published immediately on the blockchain. 
The benefit is that off-chain transactions can be updated many times before published to the blockchain resulting in reduced on-chain transactions and ultimately less fees.
In \cite{BTC:duplex}, channels can be created unidirectional or in duplex and transactions can be updated so that the final channel balances are guaranteed to be included. 
This is accomplished by newer transactions having smaller timelocks than earlier transactions and thus being able to be published sooner than old invalidated transactions. 
A limitation to this approach is that channels will have some finite life.
References \cite{BTC:lightning} and \cite{ETH:Raiden} allow for channels to remain open indefinitely or until the owners decide to close the channel. 
As distributed energy resources such as solar, storage technology, and wind power become more prevalent in the modern electric power grid, it is possible for end users to produce more energy than they consume at various times of the day.
Therefore a payment protocol for AMI should allow for bidirectional payments. 


In these solutions, transactions are properly formatted so that either party involved can post the transaction at anytime to the blockchain in case of dispute.
This property allows for the protocol to remain trustless.
The advantage to this is that the transaction can be updated off-chain to reflect a new balance and only published upon closure to the blockchain avoiding the problem of excessive fees.
Therefore this solution has the benefit that fees only need to be paid when opening and closing a channel and updating the balance within the channel is fee-less.

The major challenge in off-chain transactions is when updating the channel balance by creating a new transaction, the old unpublished transactions need to be invalidated. 
In \cite{BTC:lightning}, the Lightning Network, this is accomplished by using Revocable Delivery Transactions which are designed using timelocks and Bitcoin Scripts that enable users to forfeit funds if they publish old channel states to the blockchain.
Correct behavior is ensured through the assumption that actors are economically rational.
The Lightning Network ensures that if an actor misbehaves they can not end up any better off than if they follow the protocol.
The natural limitation to the lightning network is that the channel participants need to have access to the blockchain to follow the protocol correctly. 
If one party does not have access to the blockchain the counterparty may be able to steal funds by publishing old channel states. 
The parties need to watch the blockchain to ensure that if an old state is published that they take appropriate actions.

Because smart meters are resource limited, it is infeasible to assume that they can remain connected to the blockchain. 
Therefore we need to adopt the state channel model to allow for one (or both) parties to be offline from the Bitcoin blockchain.
In our work we assume that the smart meters have networking capability to untrusted third parties. 
By providing financial incentive third parties, the smart meters do not need to have direct access to the blockchain and can instead rely on the untrusted third parties to act as a bridge to ensure correct operation of the protocol.

The overview of the protocol is as follows, for each smart meter $SM$ the utility provider $UP$ creates a payment channel. 
Both the $UP$ and $SM$ generate 3 sets of $j$ keypairs $(pk_{\_\{UP|SM\}\_j\_\{a|b|c\}},sk_{\_\{UP|SM\}\_j\_\{a|b|c\}})$ such that each intermediate transaction -- state of payment channel -- uses a different keypair making $j$ the number of intermediate states. 
Additionally, a keypair for opening and closing the channel, $(pk_{\_\{UP|SM\}\_\{FT|close\}},sk_{\_\{UP|SM\}\_\{FT|close\}})$, and another pair for the $SM$ transacting with the third parties, $(pk_{\_DM\_3rd\_\{a|b\}},sk_{\_DM\_3rd\_\{a|b\}})$.
BIP32 \cite{BTC:bip32}, provides a deterministic hierarchical key generation algorithm and data structure that is also highly compact which minimizes the smart meters' memory requirements greatly.
All keys can be generated with a master key given a index in the data structure. 
Effectively this enables the storing of an index in place of a keypair.

The two parties agree to place a Funding Transaction $T_{FT}$ on the blockchain that sends $\sigma_{SM}$ and $\sigma_{UP}$ as input funds from $SM$ and $UP$ respectively that can be traded in the channel the output of the channel is a 2-of-2 multi-signature requiring both $SM$ and $UP$'s $sk_{\{UP|UP\}\_FT}$ to spend. 
Additionally the two parties agree on a transaction $T_{C1}$ that is valid spending the funds from $T_{FT}$ as input and returning $\sigma_{SM}$ and $\sigma_{UP}$ as output. 
Note this transaction is not published to the blockchain, its purpose is to denote the starting balance on the blockchain. 
Reference \cite{BTC:lightning} shows how two transactions, $T_{C1\_UP}$ and $T_{C1\_SM}$ can be constructed so that $UP$ is the only party that can publish $T_{C1\_SM}$ and $SM$ is the only party that is able to publish $T_{C1\_UP}$. 
This mechanism is accomplished by supplying one of the 2-of-2 input signatures required to spend $T_{FT}$'s output -- partially signing the transaction.

\todo{stuff}

The transactions $T_{C1\_UP}$ and $T_{C1\_SM}$ are made revocable by encumbering the outputs of the corresponding party's ability to send the output. For example if $SM$ publishes $T_{C1\_UP}$, the output of$\sigma_{UP}$ can be redeemed immediately by $UP$ however $\sigma_{SM}$ funds are locked.
There are two ways to redeem the locked funds, the first is for a 2-of-2 multi-signature using $SM$ and $UP$'s secret keys $sk_1$s.
The second is a timelock redeeming the funds to $SM$ after $W$ blocks. 
The first mechanism is a way for $UP$ to \textit{steal} all of $SM$s funds after both parties update the state of the channel to new transactions $T_{C2\_UP}$ and $T_{C2\_SM}$. Upon updating, $SM$ sends $sk_1$ to $UP$ (and $UP$ sends $sk_1$ to $SM$).
The \textit{stealing} of funds is the mechanism that ensures that \textit{old} transactions are not published. 
As long as $UP$ checks the blockchain before $W$ blocks after $T_{C1\_UP}$ is published, $UP$ can prevent old transactions from being published. 
This mechanism is a way to ensure that both parties follow the protocol even if the two parties do not trust each other. 

However, since the smart meters are assumed not to have direct access to the blockchain, two disjoint groups of untrusted 3rd parties are used.
Each group has multiple members to prevent collusion with the $UP$
The first group is used to publish a transaction to the blockchain incentivized through a small fee as an output to the transaction.
The second group ensures that if the $UP$ publishes an old transaction that the smart meter is notified of the transaction and is able to spend the transaction output before the timelock expires for the $UP$ to redeem their funds. 
This second group is incentivized through small fees in Bitcoin smart contracts.
In order to prevent third parties colluding with each other or the $UP$ the number of members in each third party has to be chosen with respect to the quantity of fees as well as to the channel balances.

We show later \todo{add fee analysis and protocol security} how this is done.

When both parties agree on the closing of a channel they can create a new transaction $T_{Fin}$ that uses $\sigma_{SM\_fin}$ and $\sigma_{UP\_fin}$
as the final output balances and post it to the blockchain.
If both parties follow the protocol properly, there are only two transactions published to the blockchain, $T_{FT}$ and $T_{Fin}$.
If one party tries to publish an old state of the channel $T_{Ci\_(UP/SM)}$, the other party can detect this and take all the funds in the channel. 

We now formalize the protocol and Bitcoin Scripts used to provide a real-time payment channel for smart meter real-time usage data.



\begin{figure*}
\centering
\procedure{Real-time Data Reporting and Billing Protocol}{%
\textbf{Smart Meter} \< \< \textbf{Utility Provider}  \pclb
\pcintertext[dotted]{ Channel Open } \\
KGen(), \sigma_{SM}, \sigma_{UP}, G, tx\_id_{SM}  \<\< KGen(), \sigma_{SM}, \sigma_{UP}, G, tx\_id_{UP} \\
\< \sendmessageright*{pk_{SM}} \< \\
\< \sendmessageleft*{pk_{UP}} \< \\
\text{compute } in_{INIT} = in(\sigma_{SM},rd_1'(pk_0,sk_0),tx\_id_{SM}) \< \< \text{compute } in_{INIT} = in(\sigma_{UP},rd_1'(pk_0,sk_0),tx\_id_{UP}) \\
T_{FUND} = T_{FT}(in_{INIT},) \\
\<\<\<\pclb
\pcintertext[dotted]{ Real-time Payment and Measurement } \\
\<\< \text{compute } \Vec{p} = \left<p_1,p_2,...,p_n \right> \\
\< \sendmessageleft*{\Vec{p}} \< \\
\text{measure } \Vec{m} = \left<m_1,m_2,...,m_n \right> \<\< \\
\text{compute } B = \sum_{i=1}^{n} (m_i p_i T_C) \<\< \\
\< \sendmessageright*{\Vec{m}, \textbf{ConUp}(B)} \< \\
\< \sendmessageleft*{P} \< \pclb
\pcintertext[dotted]{ Channel Close } \\
\<\<\< \\
\<\<\< \\
\<\<\< \\
\<\<\< \\
}
\end{figure*}







Definitions of the variables used in the following procedures and protocol:
\begin{itemize}
\item $ t_C \text{ : The interval that data is collected at}$
\item $ t_R \text{ : The interval that data is reported at} $
\item $ n = \frac{t_R}{t_C}  \text{ : The number of measurements / report interval} $
\item $ \Vec{p} = \left<p_1,p_2,...,p_n \right>$ Vector of n prices\footnote{\bitcoin \ is the unit of value in the Bitcoin blockchain that can be broken down into $10^9$ smaller units. 1 \bitcoin \ $ = 10^9$ Satoshis } in \bitcoin$  \e{-9}$
\item $ \Vec{m} = \left<m_1,m_2,...,m_n \right> \text{Vector of $n$ measurements}$
\item $T_{FT}$ : The funding transaction
\item $T_{C}$ : A Commitment transaction
\item $in_k$ : A input in a Bitcoin transaction
\item $out_k$ : A output in a Bitcoin transaction
\item $\sigma$ : A value in Satoshi ($10^{-9} \times $\bitcoin)
\item $(pk,sk)$ : A keypair 
\item $tx\_id$ : Some valid transaction ID and output index
\item $ rd $ : A redemption script which requires $rd'$ to make valid
\end{itemize}

The Funding Transaction $T_{FT}$ is a tuple consisting of inputs\footnote{There may need to be multiple inputs from a party in order to total the correct number of funds agreed upon. For simplicity we assume here only one input is needed from each party.} from the smart meter and utility provider and an output to a 2-of-2 multisignature as well as change outputs (unless the parties with to use all the redeeming funds in the channel): 
\begin{align}
T_{FT}(in_{SM}, in_{UP}, out_{MSig}, out_{SM}, out_{UP})
\end{align}

where $in_{k}$ is a tuple consisting of the source transaction ID, a redemption script (i.e., a signed public key), and the value from the tx\_id 
\begin{align}
in_k(\sigma, rd, tx\_id)
\end{align}

and $out_{k}$ is a tuple consisting of the value, a redemption script (which specifies who can redeem $\sigma$, and the value 
\begin{align}
out_k(\sigma, rd)
\end{align}

A commitment transaction is a tuple with an input which is the output of the funding transaction $T_{FT}$, and two outputs.

\begin{align}
T_C( \ &in(T_{FT}.tx\_id(), T_{FT}.rd', T_{FT}.\sigma),\\
&out_{local}(\sigma-\sigma',rd), \notag \\
&out_{remote}(\sigma',rd) \ ) \notag
\end{align}

We now define the $rd$ and $rd'$ scripts used in the input/outputs needed for our protocol. 
%For the Bitcoin syntax of the scripts we link to those in our external documents
Basically $rd$ defines a set of conditions that determine how and when an output can be used as an input into another transaction.
Most commonly in Bitcoin is an $rd$ that requires a keypair ($pk,sk$) such that the hash of the public key equals the value included in $rd$ proving knowledge of the public key, and a signature using $sk$ which proves ownership of the keypair.
The Bitcoin primitives mentioned earlier can be included to add a time restriction to the $rd$. 
Additionally IF-ELSE logic can be included to make the output conditional.
For the common $rd$ that requires knowledge of the secret key and a public key we define $rd_1$ for a given keypair ($pk,sk$). We are showing that $rd_1'$ is a function of the keypair, this function does not reveal $sk$, it creates a signature of the transaction with the private key, $Sig(sk,tx\_id)$. Therefore $rd_j'$ does not reveal the secret key but proves ownership.

\begin{align}
    isValid(rd_1(pk) , rd_1'(pk,sk)) == True
\end{align}

For $rd_2$ a 2-of-2 multisignature with given keypairs ($pk_1,sk_1$) and ($pk_2,sk_2$).
\begin{align}
    isValid(rd_2(pk_1,pk_2) , rd_2'(pk_1,pk_2,sk_1,sk_2)) \\== True \notag
\end{align}

For a timelock, $G$ denotes the block height, $isValid(G)$ returns True if the height of the current block is higher than $G$.

\begin{align}
    isValid(rd_3(pk \land G) , rd_3'(pk,sk) \land isValid(G)) \\== True \notag
\end{align}

In order to design the revocable transactions described in \cite{BTC:lightning}, we construct $rd_4$.

\begin{align}
    isValid(rd_4(rd_2 \lor rd_3) , rd_4'(rd_2' \lor rd_3')) == True 
\end{align}

It is important to point out that once an output is redeemed it can not be redeemed again, this prevents double spending.
$rd_4$ is designed to encumber funds in a timelock unless a multisignature can evaluate to True.
When a transaction is invalidated, the counterparty learns the corresponding multisignature key.
Transactions are invalidated if they are \emph{old} states of the channel.
However if the transaction is posted can only be published by the other party, making it irrational for it being published at all.

%For use in the commitments, we want an output that evaluates to true if a multisignature is 

The benefit to doing off-chain payments is that only two transactions need to be posted to the blockchain which allows for a great reduction of fees compared to the naive approach listed above.
If both parties follow the protocol then the funding transaction size is \todo{calc bytes} and the closing transaction size is \todo{calc bytes and say usd fee}
One downside to the protocol however is that payment is locked into the channel upon creation of the funding transaction. 
While funds are not prepaid (any party can close out the channel at any-time) they can not be spent elsewhere during the life of the payment channel. 
This leads to a tradeoff of how frequently to open and close new channels, the more frequent the less funds are locked up but the fees over time increase.
One solution to prevent the lockup of fees is to use the Lightning Network \cite{BTC:lightning} which supports chaining payment channels together to route funds through multiple untrusted intermediaries.
The downside of that approach is that there are additional fees paid to the intermediaries which are not standardized at this time.
Determining the interval for opening and closing channels and reducing the lockup of fees is an open question for this Bitcoin based protocol.








In \cite{blockchain:energy:1}, Aitzhan and Svetinovic propose a token based system similar to Bitcoin and coupled with an anonymous messaging system to provide security and privacy for peer-to-peer energy trading. 
They also include the ability to open unidirectional payment channels for partial payment. 
Their approach designs an anonymous market revolving around energy trading.
In our work we focus on solely on bidirectional payment channels for utility to end consumer energy payment. 

In \cite{blockchain:energy:3}, the authors focus on creating a local energy market for matching energy orders in a decentralized manner.
Their proposal is for a private or permissible blockchain which operates as a decentralized trusted application. 
In this work we focus on integrating the existing end-user to utility provider on public trustless blockchains.

In \cite{blockchain:energy:4}, the authors propose a token based smart contract that charges coins per kWh consumed and mints coins per kWh generated.
Coins can then be traded on an exchange to other currencies. 
This approach focuses on distributed generation of renewable power whereas our strategy is specifically for AMI.

In \cite{blockchain:energy:5}, Blockchain is evaluated for use in smart homes but the blockchain proposed does not use a trustless consensus algorithm which makes it a decentralized database for recording internet-of-things devices.

%In \cite{blockchain:energy:6}, coin where coin gen is tied to energy gen
In \cite{blockchain:energy:7}, the authors discuss some potential issues with with smart grid such as speed, scale and security and suggest that blockchain may help provide an answer.
They call for the need of a testbed and tools to evaluate blockchain within the electric grid.
One of the potential use cases the authors note is AMI billing which reaffirms our motivation for designing a real-time AMI billing protocol.

In \cite{blockchain:energy:8}, the authors suggest use of a permissioned private blockchain as a distributed database for devices throughout the smart grid. 
Their approach uses blocks to hold measurements to increase security but this approach does not scale as the measurements would need to be kept on each node in the network and their approach does not use any value tokens which prevents our real-time billing protocol from working.

Our approach uses the Bitcoin blockchain for our protocol design, there are many other blockchains that have useful properties such as Ethereum \cite{ETH:whitepaper} which has a shorter block time and implements a turing-complete scripting language.
However payment channels are still in development and on-chain transactions will still suffer from the high fee problem Bitcoin on-chain transactions do.
In our future work we will analyze trade-offs between blockchain ecosystems for real-time AMI payments.





While real time payments in advanced metering infrastructure is possible through blockchain based payment channels, in our future work we would like to implement the protocol to measure the performance impact and determine hardware requirements for smart meters since they have limited processing and storage abilities.
We would also like to explore the ability of privacy preserving blockchain privacy channels such as Bolt \cite{blockchain:bolt} in order to protect the rights of end-users. 
The major difficulty associated with anonymity within AMI is ensuring that utility providers can maintain the same configurability, and information assurance properties of the individual meters. 
In this paper we have analyzed real-time blockchain based payment for energy usage and shown that off-chain payment channels are feasible for AMI billing.
Real-time billing and payment in AMI networks enable the utility provider to receive payment for energy consumed as well as enabling payment for energy produced. 
Creating real-time billing matches the utilities goals of real-time pricing and can enable for smarter programmable contracts to aid in the utilities operations such as demand response.
